A Data-driven Contact Estimation Method for Wheeled-Biped Robots

Contact estimation is a key ability for limbed robots, where making and breaking contacts has a direct impact on state estimation and balance control. Existing approaches typically rely on gate-cycle priors or designated contact sensors. We design a contact estimator that is suitable for the emerging wheeled-biped robot types that do not have these features. To this end, we propose a Bayes filter in which update steps are learned from real-robot torque measurements while prediction steps rely on inertial measurements. We evaluate this approach in extensive real-robot and simulation experiments. Our method achieves better performance while being considerably more sample efficient than a comparable deep-learning baseline.

==> 0_backup.tex <==

Alternative designs have emerged to achieve efficient locomotion on uneven surfaces, such as tracked treads, actuated axles~\cite{nakajima_rt-mover_2011} and hybrid wheel designs like rimless \emph{spoke}-wheels~\cite{morrey_highly_2003} or re-configurable wheels~\cite{zheng_wheeler_2019}. Most of these designs, however, are often not as agile as legged robots yet make considerable compromises on efficiency and simplicity. Even a seemingly simple design as rimless wheels~\cite{morrey_highly_2003} would increase losses as wheel centers can no longer follow straight (and smooth) trajectories. 


At each timestep, we update the probability of contact based on the current observation $\zeta_t$ and the previous state $S_{t-1}$ using Bayesian inference. The probability of contact at time $t$ is then given by:
\begin{equation}
    P(S_t \ | \ \zeta_t, \ S_{t-1}) = \frac{P(\zeta_t, \ S_{t-1} \ | \ S_t) \ P(S_t)}{P(\zeta_t, \ S_{t-1})}. 
    \label{eq:prob_model_joint_denominator}
\end{equation}

We assume that the contact state $S_t$ depends only on the previous contact state (i.e. $P(S_t\,|\,S_{1..t-1}) = P(S_t\,|\,S_{t-1})$) and the observation $\zeta_t$ depends only on the current contact state: $P(\zeta_t \,|,\, S_t, \cdot) = P(\zeta_t \,|,\, S_t)$.
This Markov assumption allows us to factorize the denominator in \eqref{eq:prob_model_joint_denominator} and simplify the equation further as:

\begin{align}
    P(S_t\,|\,\zeta_t,\,S_{t-1}) &= \frac{P(\zeta_t,\,S_{t-1}\,|\,S_t)\,P(S_t)}{P(\zeta_t)\,P(S_{t-1})} \\
                                    &= \frac{P(\zeta_t\,|\,S_t)\,P(S_{t-1}\,|\,S_t)\,P(S_t)}{P(\zeta_t)\,P(S_{t-1})}  \\
                                    &= \frac{P(\zeta^t\,|\,S^t)\,P(S^t\,|\,S^{t-1})\,\cancel{P(S^{t-1})\,P(S^t)}}{P(\zeta^t)\,\cancel{P(S^{t-1})\,P(S^t)}}  \\
                                    &= \frac{\overbrace{P(\zeta_t\,|\,S_t)}^{\textit{measurement model}}\,\overbrace{P(S_t\,|\,S_{t-1})}^{\textit{transition model}}}{\underbrace{P(\zeta_t)}_{evidence}}. \label{eq:prob_model}
\end{align}

Note that the probability model in \eqref{eq:prob_model} is conditioned on the previous contact state $S_{t-1}$, which is unknown in practice. We therefore marginalize over the previous contact state to obtain the probability of contact at time $t$:

\begin{equation}
    P(S_t\,|\,\zeta_t) = \sum_{S \in \{C, \lnot C\}} P(S_t\,|\,\zeta_t, \ S_{t-1})\,P(S_{t-1}\,|\, \zeta_{t-1}).
    \label{eq:prob_model_marginalized}
\end{equation}

The recursive formulation above is similar to a hidden Markov model (HMM) where the hidden state is the contact state $S_t$ and the observation is the joint and inertial measurements vector $\zeta_t$. The transition model $P(S_t\,|\,S_{t-1})$ is the probability of transitioning from one contact state to another, and the measurement model $P(\zeta_t^\tau\,|\,S_t)$ is the likelihood of observing the joint measurements given the contact state.%

